Dyadic Reinforcement Learning

Mobile health aims to enhance health outcomes by delivering interventions to individuals as they go about their daily life. The involvement of care partners and social support networks often proves crucial in helping individuals managing burdensome medical conditions. This presents opportunities in mobile health to design interventions that target the dyadic relationship -- the relationship between a target person and their care partner -- with the aim of enhancing social support. In this paper, we develop dyadic RL, an online reinforcement learning algorithm designed to personalize intervention delivery based on contextual factors and past responses of a target person and their care partner. Here, multiple sets of interventions impact the dyad across multiple time intervals. The developed dyadic RL is Bayesian and hierarchical. We formally introduce the problem setup, develop dyadic RL and establish a regret bound. We demonstrate dyadic RL's empirical performance through simulation studies on both toy scenarios and on a realistic test bed constructed from data collected in a mobile health study.

==> tikz_others/DAG1.tex <==

\begin{tikzpicture}[gray node/.style={circle,fill=gray!20, draw=gray!60, very thick,minimum size=1cm,inner sep=0pt},
green node/.style={circle,fill=green!20, draw=green!60, very thick,minimum size=1cm,inner sep=0pt},
yellow node/.style={circle,fill=yellow!20, draw=yellow!80, very thick,minimum size=1cm,inner sep=0pt}
]
    \node[green node] (ST) at (6,0) {$R^T_t$};
    \node[gray node] (SC) at (0,0) {$S^C_{t-1}$};
    \node[gray node] (SD) at (3,0) {$S^D_{t-1}$};

    \node[yellow node] (AT) at (6,-2) {$A^T_t$};
    \node[yellow node] (AC) at (0,-2) {$A^C_{t-1}$};
    \node[yellow node] (AD) at (3,-2) {$A^D_{t-1}$};

    \path[->, thick, -stealth]
    (SC) edge[bend left] node {} (ST)
    (SD) edge[bend left] node {} (ST)
    (AC) edge node {} (SC)
    (AD) edge node {} (SD)
    (AT) edge node {} (ST);
    
\end{tikzpicture}

==> tikz_others/DAG_weekly.tex <==
\begin{tikzpicture}[gray node/.style={circle,fill=yellow!20, draw=brown!60, very thick,minimum size=1cm,inner sep=0pt},
red node/.style={circle,fill=red!10, draw=red!60, very thick,minimum size=1cm,inner sep=0pt},
blue node/.style={circle,fill=blue!10, draw=blue!80, very thick,minimum size=1cm,inner sep=0pt},
gray square node/.style={rectangle,fill=yellow!20, draw=brown!60, very thick,minimum size=1cm,inner sep=3pt},
blue square node/.style={rectangle,fill=blue!10, draw=blue!80, very thick,minimum size=1cm,inner sep=0pt},
green node/.style={rectangle,fill=green!10, draw=green!60, very thick,minimum size=1cm,inner sep=3pt}
]
    \node[gray square node] (SDw) at (0,0) {$S^D_w$};
    \node[gray node] (STw1) at (2,0) {$S^T_{w,1}$};
    \node[gray node] (STw2) at (3.8,0) {$S^T_{w,2}$};
    \node (STw3) at (5.1,0) {};
    \node (STw3top) at (5.4,0.2) {};
    \node  at (5.4,0) {$\dots$};
    \node (STw6) at (5.7,0) {};
    \node[gray node] (STwH) at (7,0) {$S^T_{w,H}$};
    \node[gray square node] (SDw1) at (10,0) {$S^D_{w+1}$};
    
    \node[blue node] (ATw1) at (2,1.5) {$A^T_{w,1}$};
    \node[blue node] (ATw2) at (3.8,1.5) {$A^T_{w,2}$};
    \node  at (5.4,1.5) {$\dots$};
    \node (ATw6) at (5.4,1.3) {};
    \node[blue node] (ATwH) at (7,1.5) {$A^T_{w,H}$};
    
    \node[red node] (Rw1) at (2,3) {$R_{w,1}$};
    \node[red node] (Rw2) at (3.8,3) {$R_{w,2}$};
    \node  at (5.4,3) {$\dots$};
    \node[red node] (RwH) at (7,3) {$R_{w,H}$};
    
    \node[blue square node] (ADw) at (1,-2) {$A^D_w$};
    \node[blue square node] (ADw1) at (11,-2) {$A^D_{w+1}$};
    \node[gray node] (STw11) at (12,0) {$S^T_{w+1,1}$};
    \node[blue node] (ATw11) at (12,1.5) {$A^T_{w+1,1}$};
    \node[red node] (Rw11) at (12,3) {$R_{w+1,1}$};
    \node  at (13,0) {$\dots$};
    \node  at (13,1.5) {$\dots$};
    \node  at (13,3) {$\dots$};

    \node  at (0,3.5) {Week $w$};
    \node  at (10,3.5) {Week $w+1$};
    
    \path[->, thick, -stealth]
    (ADw) edge node {} (STw1.south)
    (ADw) edge node {} (STw2.south)
    (ADw) edge node {} (STwH.south)
    
    (ATw1) edge node {} (Rw1)
    (ATw2) edge node {} (Rw2)
    (ATwH) edge node {} (RwH)
    
    (STw1) edge[bend right] node {} (Rw1)
    (STw2) edge[bend right] node {} (Rw2)
    (STwH) edge[bend right] node {} (RwH)

    (STw1) edge node {} (STw2)
    (STw2) edge node {} (STw3)
    (STw6) edge node {} (STwH)
    
    (ATw1) edge node {} (STw2)
    (ATw2) edge node {} (STw3top)
    (ATw6) edge node {} (STwH);


    \node[green node] (dental) at (10,6) {Dental Health};
    \path[gray!60, ->, thick, -stealth]
    (Rw1) edge node {} (dental)
    (Rw2) edge node {} (dental)
    (RwH) edge node {} (dental)
    (Rw11) edge node {} (dental);

    \path[->, thick, -stealth]
    (ADw1) edge node {} (STw11.south)  
    (ATw11) edge node {} (Rw11) 
    (STw11) edge[bend right=37] node {} (Rw11);


    \node (aboveSDw) at (0.8,2.1) {};
    \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (Rw1.south west)};

    \node (aboveSDw) at (1.2,2.1) {};
    \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (Rw2.south west)};

    \node (aboveSDw) at (1.7,2) {};
    \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (RwH.south west)};

    \path[->, thick, -stealth]
    (SDw1) edge[bend left] node {} (Rw11);
    
\end{tikzpicture}

==> tikz_others/DAG_weekly1.tex <==
\usetikzlibrary{bayesnet}

\begin{tikzpicture}[gray node/.style={circle,fill=yellow!20, draw=brown!60, very thick,minimum size=1cm,inner sep=0pt},
red node/.style={circle,fill=red!10, draw=red!60, very thick,minimum size=1cm,inner sep=0pt},
blue node/.style={circle,fill=blue!10, draw=blue!80, very thick,minimum size=1cm,inner sep=0pt},
gray square node/.style={rectangle,fill=yellow!20, draw=brown!60, very thick,minimum size=1cm,inner sep=3pt},
blue square node/.style={rectangle,fill=blue!10, draw=blue!80, very thick,minimum size=1cm,inner sep=0pt},
green node/.style={rectangle,fill=green!10, draw=green!60, very thick,minimum size=1cm,inner sep=3pt}
]
    \node[gray square node] (SDw) at (-0.5,0) {$S^D_w$};
    \node[blue square node] (ADw) at (-0.5,1.5) {$A^D_w$};
    \node[gray node] (STw1) at (2,0) {$S^T_{w,1}$};
    \node[gray node] (STw2) at (3.8,0) {$S^T_{w,2}$};
    \node (STw3) at (5.1,0) {};
    \node (STw3top) at (5.4,0.2) {};
    \node  at (5.4,0) {$\dots$};
    \node (STw6) at (5.7,0) {};
    \node[gray node] (STwH) at (7,0) {$S^T_{w,H}$};
    \plate [inner sep=2pt, yshift=3pt, dashed, thick] {plateS} {(STw1)(STwH)} {};
    
    \node[blue node] (ATw1) at (2,1.5) {$A^T_{w,1}$};
    \node[blue node] (ATw2) at (3.8,1.5) {$A^T_{w,2}$};
    \node  at (5.4,1.5) {$\dots$};
    \node (ATw6) at (5.4,1.3) {};
    \node[blue node] (ATwH) at (7,1.5) {$A^T_{w,H}$};
    
    \node[red node] (Rw1) at (2,3) {$R_{w,1}$};
    \node[red node] (Rw2) at (3.8,3) {$R_{w,2}$};
    \node  at (5.4,3) {$\dots$};
    \node[red node] (RwH) at (7,3) {$R_{w,H}$};
    \plate [inner sep=2pt, yshift=3pt, dashed, thick] {plateR} {(Rw1)(RwH)} {};
    
    
    \node[gray square node] (SDw1) at (9.7,0) {$S^D_{w+1}$};
    \node[blue square node] (ADw1) at (9.7,1.5) {$A^D_{w+1}$};
    \node[gray node] (STw11) at (12,0) {$S^T_{w+1,1}$};
    \node[blue node] (ATw11) at (12,1.5) {$A^T_{w+1,1}$};
    \node[red node] (Rw11) at (12,3) {$R_{w+1,1}$};
    \node (STw11dots) at (13,0) {$\dots$};
    \node  at (13,1.5) {$\dots$};
    \node (Rw11dots) at (13,3) {$\dots$};
    \plate [inner sep=2pt, yshift=3pt, dashed, thick] {plateS1} {(STw11)(STw11dots)} {};
    \plate [inner sep=2pt, yshift=3pt, dashed, thick] {plateR1} {(Rw11)(Rw11dots)} {};

    \node  at (0,3.5) {Week $w$};
    \node  at (10,3.5) {Week $w+1$};
    
    \path[->, thick, -stealth]
    % (ADw) edge node {} (STw1.south)
    % (ADw) edge node {} (STw2.south)
    % (ADw) edge node {} (STwH.south)
    
    (ATw1) edge node {} (Rw1)
    (ATw2) edge node {} (Rw2)
    (ATwH) edge node {} (RwH)
    
    (STw1) edge[bend right] node {} (Rw1)
    (STw2) edge[bend right] node {} (Rw2)
    (STwH) edge[bend right] node {} (RwH)

    (STw1) edge node {} (STw2)
    (STw2) edge node {} (STw3)
    (STw6) edge node {} (STwH)
    
    (ATw1) edge node {} (STw2)
    (ATw2) edge node {} (STw3top)
    (ATw6) edge node {} (STwH);


    \node[green node] (dental) at (10,6) {Dental Health};
    \path[gray!60, ->, thick, -stealth]
    (Rw1) edge node {} (dental)
    (Rw2) edge node {} (dental)
    (RwH) edge node {} (dental)
    (Rw11) edge node {} (dental);

    \path[->, thick, -stealth]
    %(ADw1) edge node {} (STw11.south)  
    (ATw11) edge node {} (Rw11) 
    (STw11) edge[bend right=37] node {} (Rw11);


    % \node (aboveSDw) at (0.8,2.1) {};
    % \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (Rw1.south west)};

    % \node (aboveSDw) at (1.2,2.1) {};
    % \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (Rw2.south west)};

    % \node (aboveSDw) at (1.7,2) {};
    % \draw[->, thick, -stealth] plot[smooth] coordinates {(SDw.north) (aboveSDw) (RwH.south west)};
    \path[->, thick, -stealth]
    (SDw) edge node {} ([yshift=-10pt] plateR.west)
    (SDw) edge node {} (plateS.west)
    (ADw) edge node {} (plateR.west)
    (ADw) edge node {} ([yshift=10pt] plateS.west);
    

    \path[->, thick, -stealth]
    (SDw1) edge node {} ([yshift=-10pt] plateR1.west)
    (SDw1) edge node {} (plateS1.west)
    (ADw1) edge node {} (plateR1.west)
    (ADw1) edge node {} ([yshift=10pt] plateS1.west);
    
\end{tikzpicture}

==> tikz_others/information_flow1.tex <==

\begin{tikzpicture}[gray node/.style={circle,fill=gray!20, draw=gray!60, very thick,minimum size=1cm,inner sep=0pt},
green node/.style={circle,fill=green!20, draw=green!60, very thick,minimum size=1cm,inner sep=0pt},
yellow node/.style={circle,fill=yellow!20, draw=yellow!80, very thick,minimum size=1cm,inner sep=0pt},
text node blue/.style={rectangle,fill=blue!20, draw=blue!80, very thick,minimum size=1cm,inner sep=5pt},
text node red/.style={rectangle,fill=red!20, draw=red!80, very thick,minimum size=1cm,inner sep=5pt}
]
    \node[green node] (ST) at (6,0) {$R^T_t$};
    \node[gray node] (SC) at (0,0) {$S^C_{t-1}$};
    \node[gray node] (SD) at (3,0) {$S^D_{t-1}$};

    \node[yellow node] (AT) at (6,-2) {$A^T_t$};
    \node[yellow node] (AC) at (0,-2) {$A^C_{t-1}$};
    \node[yellow node] (AD) at (3,-2) {$A^D_{t-1}$};

    \node[text node red] (manager) at (3,2) {Manager Agent};
    \node[text node blue] (worker) at (3,-4) {Worker Agent};

    \node  at (3,-1) {Environment};

    \path[->, thick, dashed, -stealth]
    (SC) edge node {} (manager)
    (SD) edge node {} (manager)
    (ST) edge node {} (manager);

    \path[->, thick, -stealth, draw=blue!80]
    (worker) edge node {} (AC)
    (worker) edge node {} (AD);

    \draw[->,rounded corners, thick, draw=red!80] (manager) -| node{} ++ (-5,-3) |- (worker);
    \draw[->,rounded corners, thick, draw=red!80] (manager) -| node{} ++ (5,-2) |- (AT);

    \draw[draw=gray, rounded corners, thick, fill=white!80!black, opacity=0.2]
    (-1,-2) |- (3,1) -| (7,-2) |- (3,-3) -| (-1,-2);

    \node[circle,fill=red!20, draw=red!80, very thick,minimum size=1cm,inner sep=0pt]  at (-2,-1) {$\tilde{R}_t$};
    
\end{tikzpicture}

==> tikz_others/social_network_tikz1.tex <==

\begin{tikzpicture}[red square node/.style={rectangle,fill=red!20, draw=red!60, very thick,minimum size=1cm,inner sep=0pt},
blue square node/.style={rectangle,fill=blue!20, draw=blue!60, very thick,minimum size=1cm,inner sep=0pt}]
    \node[red square node] (T) at (6,0) {$T$};
    \node[red square node] (C) at (0,0) {$C$};
    \node[blue square node] (D) at (3,0.8) {$D$};
    \coordinate (M) at (3,0);
    \node at (6,1) {Target Person};
    \node at (0,1) {Care Partner};
    \node at (3,1.8) {Dyad};

    \path[draw,thick]
    (T) edge node {} (C)
    (M) edge node {} (D);
\end{tikzpicture}
